AUGUST: an Automatic Generation Understudy for Synthesizing Conversational Recommendation Datasets

High-quality data is essential for conversational recommendation systems and serves as the cornerstone of the network architecture development and training strategy design. Existing works contribute heavy human efforts to manually labeling or designing and extending recommender dialogue templates. However, they suffer from (i) the limited number of human annotators results in that datasets can hardly capture rich and large-scale cases in the real world, (ii) the limited experience and knowledge of annotators account for the uninformative corpus and inappropriate recommendations. In this paper, we propose a novel automatic dataset synthesis approach that can generate both large-scale and high-quality recommendation dialogues through a data2text generation process, where unstructured recommendation conversations are generated from structured graphs based on user-item information from the real world. In doing so, we comprehensively exploit: (i) rich personalized user profiles from traditional recommendation datasets, (ii) rich external knowledge from knowledge graphs, and (iii) the conversation ability contained in human-to-human conversational recommendation datasets. Extensive experiments validate the benefit brought by the automatically synthesized data under low-resource scenarios and demonstrate the promising potential to facilitate the development of a more effective conversational recommendation system.

==> body/old/exp.tex <==
\input{body/tab/distn}
\begin{figure}[t]
\centering 
\includegraphics[width=0.47\textwidth]{body/fig/case_study.pdf}
\caption{Visualization of a generation case by AUGUST.} 
\label{Fig.case} 
\end{figure}

\input{body/tab/auto_eval}
\section{Experiments}
% In this section, we first set up the experiments, and then report the results and analysis.
\subsection{Experiment Setting}
\subsubsection{Resources}
% MovieLens, ReDial, Dbpedia
\textbf{(1) The ReDial dataset}~\cite{li2018towards} is collected by crowd-sourcing users on Amazon Mechanical Turk (AMT). Two paired workers serve as the recommender and user to produce a conversation and cover at least 4 different movies. Every movie mentioned in the dialog is annotated explicitly. 
\textbf{(2) The MovieLens} dataset~\cite{harper2015movielens}, released by GroupLens Research, describes people's expressed preferences for movies. These preferences take the form of $<$user, item, rating, time-stamp$>$ tuples, where the rating (1$\sim$5) represents the user's preference for a movie at a particular time. These preferences are collected by the MovieLens website, a recommender system that asks its users to give movie ratings for personalized movie recommendations. 
\textbf{(3) The DBpedia knowledge base}~\cite{auer2007dbpedia} contains structured knowledge extracted from Wikipedia. It collects rich movie-related information and inter-movie relations and releases an open knowledge graph available to the public. % A knowledge graph is a special kind of database which stores knowledge in a machine-readable form and provides a means for information to be collected, organised, shared, searched, and utilised. 

\subsubsection{Datasets}
To evaluate the performance of our methods on Graph2Dialogue and general Data2Text generation tasks, we conduct experiments on three datasets including ReKG2D, MLKG2D, and WebNLG~\cite{gardent2017webnlg}. Each sample consists of an input graph formed by triples and a target text in the form of sentences or dialogues along with a mapping from entity mentions to corresponding KG entities.  The training instances in ReKG2D and MLKG2D are both graph-dialogue pairs reformalized from the ReDial dataset,  while the test instances of ReKG2D and MLKG2D are Graph-Dialogue pairs generated from ReDial and MovieLens, respectively. For evaluation, we asked human annotators to write 100 conversations based on triples sampled from MovieLens as the generation targets. WebNLG is a popular benchmark for a general Data2Text generation task, which contains less input triples and shorter target text compared with ReKG2D and MLKG2D. 



%Table \ref{}shows the statistics for the generated dataset.
\subsubsection{Evaluation Metrics}
To investigate the performance of various methods on the Data2Text generation task, we first conduct evaluation on the quality of \textbf{conversation reconstruction}. We adopt four automatic evaluation metrics widely used in Data2Text generation tasks~\cite{li2021few}: BLEU~\cite{papineni2002bleu} and ROUGE-L~\cite{lin2004rouge}, which computes the overlap ratio of $n$-grams between the reconstructed dialogue and the original one; CIDEr~\cite{vedantam2015cider} that computes the TF-IDF weights for each $n$-gram in synthetic/real dialogues; and Chrf++~\cite{popovic2017chrf++} that computes the average F-score on both character-level and word-level $n$-grams. 
For the \textbf{conversation writing} quality, we compute Dist-$n$~\cite{li2015diversity} to show the distinctness of the generated utterances and the perplexity (PPL) proposed in \cite{jelinek1977perplexity} to measure the language fluency. Besides, we also conduct human evaluation to show the generation quality following the previous works in \cite{li2021few, agarwal2021knowledge}, which contains three workers' ratings to 200 randomly sampled dialogues with respect to fluency, grammar, dialogue logic, and informativeness. 
% we conduct human evaluation in addition to automatic evaluation, we randomly sample 200 KG subgraphs along with corresponding generated text from baseline models and our model. Three workers were asked to score the text with respect to two aspects: Factual correctness and Language naturalness to evaluate how well the generated conversation correctly conveys information contained in the KG and how well the generated conversation is grammatically correct and fluent.

%\subsubsection{Models in this study}
%We investigate BART \cite{lewis2020bart} and T5 \cite{raffel2020exploring}, two PLMs based on the Transformer encoder-decoder architecture \cite{vaswani2017attention} for graph-to-conversation generation as previous works \cite{ribeiro2021investigating,li2021few} on graph-to-text generation tasks. 
%To evaluate various models' performance on generating conversation from the given graph, We chose to explore and compare Transformer, Pointer Generator, BART, T5, and our model's performance on data-to-text generation task.

\subsubsection{Implementation Details}
\label{sec:imp}
For the graph encoder in AUGUST, we use a two-layer R-GCN with an embedding size of 1,024. As for the text decoder, we investigate two versions, base and large, of Bart~\cite{lewis2020bart} for dialogue generation. We optimize all parameters with an AdamW~\cite{loshchilov2017decoupled} optimizer with a learning rate of $10^{-5}$. The weight factors, $\lambda_1$, $\lambda_2$, and $\lambda_3$ are set to 0.8, 0.8, and 0.1, respectively. The whole network is trained on 4$\times$23GB NVIDIA Tesla P40 with a  minibatch size of 16. 
%\cite{schlichtkrull2018modeling}
%settings hyper-parameters


\subsection{Experiment Results}
\subsubsection{Evaluation}
We give both automatic and human evaluations of the generation results by AUGUST. For automatic evaluation, we implement AUGUST with two versions of PLM, Bart-base and Bart-large, on all three datasets to construct a benchmark for future related works. As shown in Tab.~\ref{tab:auto_eval}, Bart-large performs better than Bart-base consistently over all datasets and metrics, which may result from more external knowledge contained in the larger PLM. With the same training data, PLM performs poorer on MLKG2D than on ReKG2D, which demonstrates the domain gap between the real and synthetic domain. Besides, the PPL value is low on all settings, so the generation has high confidence, which may result from the consistency of the generation objective between Bart pre-training and Data2Text training. Performances on WebNLG are higher than on  the other two over all metrics except PPL, because the target text in WebNLG is usually shorter and with richer common entities, and the input has fewer triples, which reduces the generation difficulty. 
Considering there is no standard answer for the generation task, automatic evaluation makes limited demonstration for the generation. Thus, we further introduce human evaluation for the generation results by AUGUST and human-labeled dialogues from the ReDial dataset. The human evaluation is conducted on two aspects: (i) Factual Correctness, \eg~the recall of input entities or relations; (ii) Language Naturalness, including expression logic, fluency, grammar accuracy, and informativeness. As presented in Tab.~\ref{eva:human}, the full score for all metrics is 5, and AUGUST implemented with Bart-large performs slightly better than with Bart-base in factual correctness. With respect to the language naturalness, impressively, generations from AUGUST are of comparable quality with samples from the ReDial dataset, which shows the great potential of automatic generation for CR datasets. 









\subsubsection{Ablation Study}
We conduct ablative experiments to validate the effect of each component, \ie, representation alignment (RA), domain adaptation (DA), and copy mechanism (CP), which correspond to three loss items, \ie, $L_{align}$, $L_{adv}$, and $L_{copy}$, respectively. The basic model is implemented with Bart-large, and all variants are evaluated on the ReKG2D test set over five metrics. As shown in Tab.~\ref{ablation}, the performance drops over almost all metrics without any of the components. Specifically, suppressing the RA component has a relatively small influence on the performance; the DA component mainly contributes to the ROUGE metric, which measures the quality of recovery compared with the reference; and the CP component can significantly affect CIDEr, Chrf, and Recall, which shows the importance of forcing the model to include the input items in generation. 

\input{body/tab/human_eval}
\input{body/tab/ablation}

%\subsubsection{Case Study}

\subsubsection{Error Analysis}
We summarize three types of errors that appeared in our generation according to the hierarchy of the dialogue requirement, with one example shown in Fig.~\ref{Fig.case}.
\textbf{Error Type I: Format Errors}, including grammar and spelling mistakes, or the unexpected writing format, \eg, each utterance is expected to start with the identity of ``[U] says:", while it may generate ``[U] thinks".
% the problem that a system generates text which say things are not true, or at least are not in the input data. Specifically, it can be i) a wrong relation between two mentioned entities, (\eg, the truth in the given input triples is that the``Seeker" doesn't like the movie "the Matrix" yet  the "Seeker" shows a fondness for ``the Matrix" in the generated dialogues, since the lack of fine-grained mappings between input triples and the conversation); ii) missing mention of one or several entities from the given input; iii) wrong reference to an entity that is not in the input; iv) wrong description of an entity (\eg, generate wrong genre, director, or synopsis of a movie).
\textbf{Error Type II: Hallucination}, which is a common problem in language generation tasks. It means the network (i) generates contents that conflict with the input data, \eg~producing wrong relations, entities, or sentiments, or (ii) generates extra items beyond the input, which means the output is not a precise description to the input, \eg~``Hancock (2008)'' in Fig.~\ref{Fig.case}. 
\textbf{Error Type III: Incoherent Logic}, which refers to the problem of incoherent  or contradictory logic in the generated dialogue, \eg~the user says (s)he has not seen a movie but liked it.  








% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}





    


==> body/old/huamn_eval_old.tex <==
\begin{table}[]
\setlength{\tabcolsep}{1.1mm}{
\begin{tabular}{l|c|cccc}
\toprule
\multirow{2}{*}{\textbf{Data}} & \small \textbf{Factual} & \multicolumn{4}{c}{Language Nat.}    \\ 
\cmidrule(lr){3-6}
& \small \textbf{Correct.} & \small \textbf{Logic} & \small \textbf{Fluency} & \small \textbf{Gram.} & \small \textbf{Inform.} \\ \midrule
\small{AUGUST} & 2.7 & 4.2 & 4.4 & 4.0 & 3.9\\
ReDial         &   - & 4.4 & 4.6 & 4.6 & 4.0\\
\bottomrule
\end{tabular}}
\caption{Human evaluation of generation by AUGUST. ``Gram.'' and ``Inform.'' means grammar and informativeness, respectively.}
\label{eva:human}
\end{table}

==> body/old/method.tex <==
\begin{figure*}[htbp]%H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.7\textwidth]{body/fig/method.pdf}%插入图片，[]中设置图片大小，{}中是图片文件名
\caption{The overview of the proposed automatic recommendational dialogue generation framework. } %最终文档中希望显示的图片标题
\label{Fig.method} %用于文内引用的标签
\end{figure*}
\section{Methodology}
%介绍训练集和测试集构造方法，以及构造过程中的策略
%介绍我们提出的一种evaluation metric作为辅助
\subsection{Preliminaries}
Our CR dataset synthesis approach produces recommendational dialogues from three kinds of resources: user-item matrices from traditional recommendation datasets, external knowledge graphs, and existing CR datasets. We first introduce related notations. \textbf{A user-item matrix} (UIM) $\mathbf{M}$ (supplied by datasets like MoviLens~\cite{harper2015movielens}) consists of $N$ rows and $M$ columns, of which the $n$-th row represents the ratings of the $n$-th user $\mathrm{U}_n$ towards all $M$ items, and each element $s_{ij} \in [1, 2, 3, 4, 5]$ represents the $n$-th user's rating score towards the $i$-th item $o_j$, where a higher score represents the user's more favor to one item. Note that the matrix $\mathbf{M}$ may be sparse depending on the number of ratings given by each user. 
\textbf{A knowledge graph} $\mathbf{G} = <\mathcal{E}, \mathcal{R}>$, \eg~DBpedia~\cite{auer2007dbpedia}, where $\mathcal{E}$ and $\mathcal{R}$ are the entity and relation set, respectively. The graph consists of large amounts of entity-relation-entity triples $(e_i, r_{ij}, e_j)$, of which $e_{i}$ or $e_{j}$ can be an item or non-item entity from $\mathcal{E}$ and $r_{ij} \in \mathcal{R}$ represents the relation category between an associated entity pair. We denote the item entity set as $\mathcal{O} \subset \mathcal{E}$, which contains all recommendation candidates. 
In \textbf{a CR dataset} (\eg~ReDial~\cite{liu2020towards}), a conversation is generated for recommendations on various domains (movie, traveling, restaurant, etc.) in a seek-recommender pair. Denote the $i$-th conversation as $\mathrm{C}_i$, a seeker/user $\mathrm{U}_i$ is asking for item recommendations from a recommender $\mathrm{R}_i$. In the following chatting turns, $\mathrm{U}_i$ may express his/her preferences explicitly or implicitly, then $\mathrm{R}_i$ is expected to capture the user's preferences according to the historical dialogue context, denoted as $\mathcal{C}_t=\{c_j\}_{1}^t$, where $t$ is the historical turn number and $c_j$ is the $j$-th conversation utterance. %At the (t−1)(t-1)-th turn, one should produce the next utterance ctc_{t} to reply the other. The reply of Ri\mathrm{R}_i can cover one or several candidate items {oj}\{o_j\} selected from the entire item set O\mathcal{O} or ask other attributes of items according to the strategy. %note that Ot=O1t,…,OTt\mathcal{O}_t = {O_t^1,\dots, O_t^T} can be equal to \empty\empty when there is no need to recommendation. In such a case, then hih_i may raise a clarification question or generate a chit-chat response.   

\subsection{Dataset Synthesis}
The proposed dataset synthesis approach starts from accurate user preferences information easily accessed from the UIM $\mathbf{M}$. Then a UIM-Graph-Dialogue generation pipeline is adopted to synthesize recommendation dialogues, with the overview shown in Fig.~\ref{Fig.method}. 

\paragraph{UIM $\rightarrow$ Graph}
The first step is to convert UIM that contains user preferences into graphs. From any row $i$ of $\mathbf{M}$, a set of items with respective ratings $\{(o_j, s_{ij})\}$ can be taken to generate a dialogue sample. All $o_j$s are used as nodes to construct the graph $\mathbf{G}'_i$. To integrate the user preferences into $\mathbf{G}'_i$, an extra node of user $u_i$ with its relation to each item node are added to constitute triples like $(u_i, s_{ij}, o_j)$ for item $o_j$. Furthermore, we extend $\mathbf{G}'_i$ by incorporating rich external knowledge from $\mathbf{G}$ for the informativeness of the final dialogue output. Specifically, for each two items $o_j$ and $o_k$, we search for an two-hop path in $\mathbf{G}$ to find their relations, \textit{i.e.}, two movies are directly linked (neighbouring) as $(o_j, r_{jk}, o_k)$ (\eg~belong to one movie series) or linked by one entity $e_l$ as $(o_j, r_{jl}, e_l, r_{lk}, o_k)$ (\eg~sharing the same director, actors, or genre). Then, these triples in the searched path are added into $\mathbf{G}'_i$. The obtained graph $\mathbf{G}'_i$ can better represent the selected items from UIM data by incorporating both accurate user-preference information and knowledge-equipped inter-entity relations. 

\paragraph{Graph $\rightarrow$ Dialogue}
Given a graph $\mathbf{G}'_i$ that represents the items expected to appear in the dialogue, a Data2Text generator aims to synthesize a conversational dialogue $\mathrm{C}_i$ based on the graph. We cast it as a Data2Text problem. We adopt a Data2Text generator to take the graph as input, and output raw text that contains the vertex and edge information in the graph. Note that two tokens [U] (user) and [R] (responder) are specially defined to be generated in the text, such that the sentences after [U] ([R]) and before the next token [R] ([U]) can be viewed as a single turn. In this way, the text can be decomposed and re-organized into a multi-turn dialogue. Considering there is no supervision (graph-dialogue data pair) for the learning of the generator in this Data2Text process, we utilize the existing CR datasets to learn a strong generator and transfer the knowledge from them into our Data2Text task, which is introduced in the following subsection.


\subsection{Domain Adaptive Data2Text Generation}
\label{data2textDA}
In order to generate both natural and logical dialogues from item-related graphs, we adopt a domain adaptive Data2Text generator to transfer the conversation knowledge learned in CR datasets to Graph $\rightarrow$ Dialogue generation, implemented with an encoder-decoder architecture as illustrated in Fig.~\ref{Fig.autoencoder}.
\paragraph{Data2Text Generator}
Given any dialogue sample $\mathrm{C}$ in existing CR datasets, we produce graph-dialogue training pairs to learn a strong Data2Text Generator. To construct the graph based on a given dialogue, we first search for all entities $\{e_j\}$ with the speaker's ($\mathrm{U}_i$ or $\mathrm{R}_i$) sentiment $\{s_{ij}\}$ to them (provided by CR datasets usually or generated from an estimator), and link each $e_j$ with corresponding nodes in $\mathbf{G}$. Then a graph $\mathbf{G}'_i$ can be constructed in a similar way as in the UIM $\rightarrow$ Graph process. In the next step, we adopt an encoder-decoder architecture for Data2Text generation. In the encoder, an R-GCN~\cite{schlichtkrull2018modeling} is applied to generate entity embeddings for $\mathbf{G}'_i$. Let $\phi_j \in \mathbb{R}^d$ denote the entity embedding for a general entity $e_j$ in KG, where $d$ is the embedding size. Then the R-GCN helps leverage the multi-relational information to have a structure-aware graph representation. Specifically, the embedding of $e_j$ at the $l+1$-th of total $L$ layers can be computed as:
$$
\phi_j^{l+1} = \sigma(\sum_{r\in\mathcal{R}}\sum_{k\in\mathcal{N}_j^r} \mathbf{W}_r^l\phi_k^l + \mathbf{W}_0^l\phi_j^l),
$$
where $\sigma(\cdot)$ is the activation function,  $\mathbf{W}_r^l$ and $\mathbf{W}_0^l$ are trainable parameters, and $\mathcal{N}_j^r$ is the set of neighbouring entities of $e_j$ under relation $r$. Note that, all $\phi_j^0$ before the first layer are initialized by pre-trained KG embeddings in \cite{yang2014embedding}. 

To learn higher-quality graph features for more smooth decoding, we leverage another encoding branch of pretrained language model (PLM) to learn context-aware node features and align ones encoded from graphs with them. Specifically, by taking the whole dialogue as PLM input, entities are represented with contextual information in natural utterances, so that rich knowledge in PLM can be adapted. The alignment between two groups of feature vectors is implemented by minimizing an l2 loss, $L_{align}$. Before feeding graph node features into the decoder, we linearize them into an entity sequence $\{\phi_j^L\}$ through a relation-biased breadth-first search (RBFS) strategy following \cite{li2021few}, where an RBFS weights are computed for each node as its score to decide the sequence order. For more related implementation details, please refer to Sec. Experiments and \cite{li2021few}. 

In the decoding stage, a PLM decoder is performed to decode the linearized graph features $\{\phi_j^L\}$ into textual dialogues. To formalize the dialogue generation into a typical natural language generation problem, we sequentially connect all utterances into a single paragraph but with special tokens as the separation for regrouping into dialogue turns.  Denote the $k$-th of total $K$ token as $w_k$, the generation objective is to minimize the negative log-likelihood as:
$$
L_{gen} = -\sum_{k=1}^K \log P(w_k | w_1, w_2, \cdots, w_{k-1}), 
$$
where $P(\cdot)$ denotes the probability function. To encourage covering entities from the input graph, a copy mechanism implemented with a pointer network is conducted, leads to a copy loss term $L_{copy}$. 

\paragraph{Adversarial Domain Adaptation}
\begin{figure}[t]%H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.4\textwidth]{body/fig/autoencoder.pdf}%插入图片，[]中设置图片大小，{}中是图片文件名
\caption{The illustration of the proposed domain adaptive encoder-decoder architecture for Data2Text generation.} %最终文档中希望显示的图片标题
\label{Fig.autoencoder} %用于文内引用的标签
\end{figure}
Although there are sufficient supervision in CR datasets (\ie, real data) to train the encoder-decoder, our synthesized data has no textual ground truths for supervised learning. Thus, we perform a domain adaptation method based on adversarial learning~\cite{lowd2005adversarial} to transfer the knowledge in the real domain to our synthesized domain. We first compute  the linearized graph features $\{\phi_r\}$ or $\{\phi_s\}$, and the text features from the last PLM decoder layer $\{\psi_r\}$ or $\{\psi_s\}$, for each sample from the real or synthesized domain, respectively. Then an adversarial learning framework is conducted to encourage both the graph encoder and PLM decoder to produce domain-invariant features, so that samples from either domain can be projected into a shared feature space to improve the robustness of encoder and decoder. Specifically, a multi-layer perceptron is implemented as the discriminator $D$, and the layers before the output layer is viewed as a generator $G$. In the adversarial training, the discriminator is forced to distinguish which domain the features come from, while the generator has the opposite objective to fuse the discriminator by generating domain-invariant features, formulated as:
$$
L_{adv} = ||D(\phi'_i) - \mathbf{I}(i)||^2 + ||D(\psi'_i) - \mathbf{I}(i)||^2, i \in \{r, s\},
$$
where $\phi'_i$ and $\psi'_i$ are the average feature vector of $\{\psi_i\}$ and $\{\psi_i\}$ from the domain $i$, respectively, $\mathbf{I}(\cdot)$ is the indication function that outputs 1 if $i$ equals to $r$ and 0 otherwise. Note that the objective is to maximize $L_{adv}$ when updating the discriminator while minimizing $L_{adv}$ when updating the generator. The overall objective function to learn the domain adaptive encoder-decoder can be written as:
$$
L_{over} = L_{gen} + \lambda_1 L_{align} + \lambda_2 L_{copy} + \lambda_3 L_{adv},
$$
where $\lambda_1$, $\lambda_2$, and, $\lambda_3$ are weight factors to balance the copy and adversarial loss, respectively.





% \paragraph{Entity Linking}
% Historical dialogue context Ct\mathcal{C}_t contains historical entities Cte=\mathcal{C}_e^t={}
% \paragraph{Subgraph Construction}
% \paragraph{Supervised Learning}
% \paragraph{Extended Reference}
% \subsection{Test Set Constructed}
% test set is used for test the ability of model generalization, and back to the beginning, we aims at training a model using deformed Redial CR data  to construct a synthesised dataset from existing user-item matrix (movielens in this work), thus it's inevitable to evaluate the quality of conversations generated from Movielens. 
% we constructed two different test dataset:
% test data separated from CRD and test data constructed from user-item matrix, for the second one, we have following steps:
% \paragraph{subgraph construction}
% \paragraph{reference construction}



% \subsection{Domain adaptation}
% \subsection{Evaluation Metrics}


==> body/old/rec_eval_old.tex <==
\begin{table*}[]
\begin{tabular}{|ll|lll|lll|lll|}
\hline
\multicolumn{2}{|c|}{MovieLensDialogue}                                                                                                  & \multicolumn{3}{c|}{0\%} & \multicolumn{3}{c|}{50\%} & \multicolumn{3}{c|}{100\%} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}data\end{tabular}} & \begin{tabular}[c]{@{}l@{}}used \\ model\end{tabular} & R@1    & R@10   & R@50   & R@1    & R@10    & R@50   & R@1    & R@10    & R@50    \\ \hline
/                                                                                & BART/KGSF                                                  &        &        &        &        &         &        &        &         &         \\ \hline
100\% Redial                                                                     & KGSF                                                  &        &        &        &        &         &        &        &         &         \\ \hline
100\% Redial                                                                     & BART                                                  &        &        &        &        &         &        &        &         &         \\ \hline
100\% AU                                                                         & KGSF                                                  &        &        &        &        &         &        &        &         &         \\ \hline
100\% AU+Re                                                                      & KGSF                                                  &        &        &        &        &         &        &        &         &         \\ \hline
100\% AU+Re                                                                      & BART                                                  &        &        &        &        &         &        &        &         &         \\ \hline
\end{tabular}
\end{table*}

==> body/old/rec_eval_vertical.tex <==
\begin{table}[]
\begin{tabular}{lllll}
data                                                           & model & Recall@1 & Recall@10 & Recall@50 \\ \hline
0\%ML                                                          & BART  &          &           &           \\
50\%ML                                                         & BART  &          &           &           \\
100\%ML                                                        & BART  &          &           &           \\ \hline
0\%ML                                                          & KGSF  &          &           &           \\
10\%ML                                                         & KGSF  &          &           &           \\
50\%ML                                                         & KGSF  &          &           &           \\ \hline
\begin{tabular}[c]{@{}l@{}}100\%Redial\\ +50\%ML\end{tabular}  & KGSF  &          &           &           \\
\begin{tabular}[c]{@{}l@{}}100\%Redial\\ +100\%ML\end{tabular} & KGSF  &          &           &           \\ \hline
\begin{tabular}[c]{@{}l@{}}100\%AU\\ +50\%ML\end{tabular}      & KGSF  &          &           &           \\
100\%AU                                                        & KGSF  &          &           &           \\
\begin{tabular}[c]{@{}l@{}}100\%AU\\ +100\%ML\end{tabular}     & KGSF  &          &           &          
\end{tabular}
\end{table}

==> body/tab/ablation.tex <==
\begin{table}[]
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{l|ccccc}
\toprule
Models     &  B-4      &  R-L     &    CIDEr  &    Chrf    &   Dist-2 \\ \midrule
Bart-large &  13.91    &  29.63   &    1.52   &    42.16   &   0.75   \\
~w/o RA    &  13.26    &  29.21   &    1.24   &    41.90   &   0.74   \\ 
~w/o DA    &  13.91    &  27.42   &    0.93   &    40.17   &   0.73   \\ 
~w/o CP    &  13.11    &  28.06   &    1.38   &    39.72   &   0.72   \\ 
~only PLM  &  12.58    &  27.43   &    1.03   &    40.33   &   0.70   \\\bottomrule
\end{tabular}}
\caption{Ablative results on ReKG2D. RA: representation alignment, DA: domain adaptation, CP: copy mechanism, only PLM: without all of the three components above.}
\label{ablation}
\end{table}
%写distinct-3 的时侯说一下是avereage的

==> body/tab/dataset.tex <==
\begin{table*}[]
\begin{tabular}{l|lllllccc}
\toprule
Datasets                              & Conv. Gen.                  & Resources                                                                & User Info.                                             & Item Info.                                                          & Guidance                                                        & R. UP & \#Dialog.        & \#Turns            \\ \midrule
TG-ReDial     & \begin{tabular}[c]{@{}l@{}}semi-autom.,\\ human verified\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}reviews, \\ user records\\ \end{tabular}         & records                                                & reviews & \begin{tabular}[c]{@{}l@{}}topic\\ thread\end{tabular}          &    \Checkmark  & 10K               & 129K               \\
COOKIE        & \begin{tabular}[c]{@{}l@{}}template,\\ human verified\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}reviews, \\ custom KG\\ \end{tabular}           & records                                                & meta-data  & \begin{tabular}[c]{@{}l@{}}key entities\\ sequence\end{tabular} &   \Checkmark   & -                 & 12M             \\
FaceBook-Rec  & template   & \begin{tabular}[c]{@{}l@{}}UIM, \\ template\end{tabular}                 & records                                                & none                                                               & QA form                                                         &   \Checkmark   & 1M                & 6M                 \\
DuRecDial     & hum.-to-hum. & \begin{tabular}[c]{@{}l@{}}user profile,\\ KG\end{tabular}               & profile                                                & KG facts                                          & \begin{tabular}[c]{@{}l@{}}goal\\ sequence\end{tabular}         &  \XSolidBrush  & 10K               & 155K               \\
DuRecDial 2.0 & hum.-to-hum. & \begin{tabular}[c]{@{}l@{}}multiligual\\ user profile,\\ KG\end{tabular} & profile                                                & KG facts                                                        & \begin{tabular}[c]{@{}l@{}}goal \\ sequence\end{tabular}        & \XSolidBrush   & 16K               & 255K               \\
OpenDialKG    & hum.-to-hum. & KG                                                                       & none                                                   & KG facts                                                        & KG path                                                         & \XSolidBrush   & 15K               & 91K                \\
MGconvRex     & hum.-to-hum.  & user profile                                                             & \begin{tabular}[c]{@{}l@{}}profile,\\ UMG\end{tabular} & none                                                           & \begin{tabular}[c]{@{}l@{}}memory \\ graph\end{tabular}         &  \Checkmark    & 7K                & 73K                \\
INSPIRED      & hum.-to-hum. & none                                                                     & none                                                   & facts                                                           & \begin{tabular}[c]{@{}l@{}}socialable\\ strategy\end{tabular}   & \XSolidBrush   & 1K                & 36K                \\
GoRecDial     & hum.-to-hum. & \begin{tabular}[c]{@{}l@{}}user profile,\\ goals, KG\end{tabular}        & records                                                & KG facts                                                        & \begin{tabular}[c]{@{}l@{}}dialogue\\ goal\end{tabular}         &   \Checkmark   & 9K                & 171K               \\
ReDial        & hum.-to-hum. & item list                                                               & none                                                   & none                                                             & instructions                                                    & \XSolidBrush   & 10K               & 182K               \\
%\midrule
\textbf{AUGUST} \textbf{(ours)} & automatic  & \begin{tabular}[c]{@{}l@{}}KG, CRD,\\ UIM\end{tabular}    & records    & KG facts  & key triples &  \Checkmark  & \textgreater{}25M  & \textgreater{}200M \\ \bottomrule
\end{tabular}
\caption{Comparison of our AUGUST with existing conversational recommendation dataset construction methods, ``Conv. Gen." stands for the conversation generation way, ``R. UP" stands for observed real user preference, ``UMG'' represents user memory graphs, and ``User Info." and ``Item Info." stand for user information and item information, respectively.}
\label{tab:datasets}
\end{table*}

==> body/tab/distn.tex <==
% \begin{table}[]
% \setlength{\tabcolsep}{2.2mm}{
% \begin{tabular}{l|cc|cc|cc}
% \toprule
% Metrics     & \multicolumn{2}{c|}{Dist-1} & \multicolumn{2}{c|}{Dist-3} & \multicolumn{2}{c}{Rec. Score}      \\ 
% \#Dialogues &  50          &  200         &  50          &  200         &  50          &  200                 \\ \midrule %\cline{1-1}
% ReDial      &  0.48        &  0.44        &  0.85        &  0.84        &   -          &  -                   \\ %\cline{1-1}
% AUGUST      &  0.48        &   0.49       &  0.84        &  0.85        &  4.98        &  4.96                \\ %\cline{1-1} 
% \bottomrule
% \end{tabular}}
% \caption{Average Dist-nn and recommendation score of randomly sampled subsets of two datasets.}
% \label{tab:dist}
% \end{table}
\begin{table}[]
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{l|cc|cc}
\toprule
Metrics     & \multicolumn{2}{c|}{Dist-1} & \multicolumn{2}{c}{Dist-3}       \\ 
\#Dialogues &  50          &  200         &  50          &  200                \\ \midrule %\cline{1-1}
ReDial      &  0.48        &  0.44        &  0.85        &  0.84                \\ %\cline{1-1}
AUGUST      &  0.48        &  0.49        &  0.84        &  0.85                \\ %\cline{1-1} 
\bottomrule
\end{tabular}}
\caption{Average Dist-$n$ and recommendation score of randomly sampled subsets of two datasets.}
\label{tab:dist}
\end{table}
